Learn Continually, Generalize Rapidly: Lifelong Knowledge Accumulation for Few-shot Learning

The ability to continuously expand knowledge over time and utilize it to rapidly generalize to new tasks is a key feature of human linguistic intelligence. Existing models that pursue rapid generalization to new tasks (e.g., few-shot learning methods), however, are mostly trained in a single shot on fixed datasets, unable to dynamically expand their knowledge; while continual learning algorithms are not specifically designed for rapid generalization. We present a new learning setup, Continual Learning of Few-Shot Learners (CLIF), to address the challenges of both learning settings in a unified setup. CLIF assumes a model learns from a sequence of diverse NLP tasks arriving sequentially, accumulating knowledge for improved generalization to new tasks, while also retaining performance on the tasks learned earlier. We examine how the generalization ability is affected in the continual learning setup, evaluate a number of continual learning algorithms, and propose a novel regularized adapter generation approach. We find that catastrophic forgetting affects generalization ability to a less degree than performance on seen tasks; while continual learning algorithms can still bring considerable benefit to the generalization ability.

==> tables/glue_cl.tex <==
\begin{table*}[]
\centering
\scalebox{0.7}{
\begin{tabular}{@{}l|rrrrrrrrr|r@{}}
\toprule
\textbf{Task}               & \textbf{CoLA} & \textbf{SST-2} & \textbf{MRPC} & \textbf{STS-B} & \textbf{QQP} & \textbf{MNLI} & \textbf{QNLI} & \textbf{RTE} & \textbf{WNLI} & \textbf{Average} \\ \midrule
\rowcolor{na}   \textit{Continual learning} &      &       &      &       &     &      &      &     &      &         \\
%{BART-LAMOL}              &      &       &      &       &     &      &      &     &      &         \\
{BART-Vanilla}              &   0.00  &   0.00     &    0.00   &   0.00    &  0.00   &   4.04   &  49.46    &   52.71   &   43.66   &    20.68  \\
{BART-MbPA++}              &   60.40  &   73.74     &    61.27   &   66.47    &  69.50   &   45.56   &  63.31    &   55.96   &   39.44   &    59.52    \\
%\addlinespace[-0.1cm]   &  \smallnum{80.15}    &    \smallnum{91.97}   &        \smallnum{80.64}    &   \smallnum{84.73}    &   \smallnum{83.25}     &    \smallnum{75.50}   &\smallnum{85.56}     &  \smallnum{58.84}    & \smallnum{56.34}      &  \smallnum{77.48}  \\

{BART-meta-MbPA}              &   30.87    &    70.41   &   68.38   &       49.53 &  67.06    &  32.75     &    76.50   &  62.09   &    43.66   &      55.69   \\
%\addlinespace[-0.1cm]            &   \smallnum{81.69}   &   \smallnum{91.62}    &   \smallnum{82.84}   &    \smallnum{85.53}   &    \smallnum{85.25}  &   \smallnum{75.94}     &    \smallnum{85.25}  & \smallnum{63.18}     &  \smallnum{56.34}    &   \smallnum{78.63}      \\
{\method-Vanilla}            & 0.00     &   49.54    &  31.37    &  49.53     &  63.18   &  0.00  &  63.92     & 70.76 &  56.34  &    42.75     \\ 
%\addlinespace[-0.1cm]                         & \smallnum{77.56}    &   \smallnum{91.74}     &  \smallnum{82.84}    &   \smallnum{85.87}    &  \smallnum{83.12}   &   \smallnum{75.03}   & \smallnum{87.33}  & \smallnum{73.64} & \smallnum{56.34}     &   \smallnum{78.68}       \\
{\method-EWC}                &   0.00   & 80.16   &  0.00    &   0.00    &  0.00   &   0.00   &   51.18   &   60.65   &   57.74    &     27.76    \\
%\addlinespace[-0.1cm]                            &   \smallnum{77.56}   & \smallnum{91.74}   &  \smallnum{73.53} &   \smallnum{83.13}    &  \smallnum{81.51}   &   \smallnum{75.42}   &  \smallnum{87.11}    &   \smallnum{70.76} &  \smallnum{57.75} &    \smallnum{73.54}     \\
{\method-Reg}               &  30.87    &   89.90    &  63.23  &    82.13   &  81.04   &  75.55  &   75.03    &   62.09    & 60.56  &    68.93     \\
%\addlinespace[-0.1cm]                            &  \smallnum{79.70}    &   \smallnum{90.94}    &   \smallnum{86.76}    &  \smallnum{85.73}    &  \smallnum{82.43}   &   \smallnum{76.22}    &  \smallnum{86.56}  &   \smallnum{69.68}  &  \smallnum{60.56}  & \smallnum{79.84}   \\
{\method$_{\backslash \textrm{ST}}$-Reg}                &   60.11    &   91.28     &    83.82   &   81.47    &  81.25   &   73.02   &   70.09   &  62.45   &    57.74   &   \textbf{73.47}  \\
%\addlinespace[-0.1cm]       &   \smallnum{78.04}    &   \smallnum{90.82}     &    \smallnum{86.52}  &    \smallnum{86.00}   &  \smallnum{81.95}   &    \smallnum{75.52}   &  \smallnum{87.06}    &  \smallnum{62.45}   &   \smallnum{57.74}   &     \smallnum{78.46}    \\
{\method$_{d=4}$-Reg}              &   78.72   &   89.68    &   31.62    &    49.80    &  78.98   &    44.38   &   57.66   &  63.54   &    59.15   &     61.50    \\
%\addlinespace[-0.1cm]       &   \smallnum{79.19}    &   \smallnum{92.43}     &    \smallnum{70.09}  &    \smallnum{83.20}   &  \smallnum{79.13}   &    \smallnum{75.83}   &  \smallnum{86.40}    &  \smallnum{70.40}   &   \smallnum{59.15}   &     \smallnum{74.01}    \\
\midrule
\rowcolor{na}  \textit{Single-task learning}   &     &       &      &       &     &      &      &     &      &         \\
{\method-Single}       &   78.52   &   90.25    &   85.54    &   85.00      &  82.31   &   75.77   &   86.40    &   53.43  &  56.34   &  \textbf{77.06}        \\
{Adapter-Single}    &  69.13   &   91.28   &   77.94   &    84.20   &  82.53   &   75.19   &  85.50  &  52.71   &   56.34   &  74.98    \\
%{BART-Single}        &      &       &      &       &     &      &      &     &      &         \\ \midrule
%{BART-MTL}           &      &       &      &       &     &      &      &     &      &         \\ 
{Majority}           &   69.13   &   50.92    &   68.38    &   50.47     &  63.18   &  35.33     &   50.54   &  52.71   &    56.34  &  55.22   \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Continual and offline learning performance on GLUE datasets evaluated at the end of the training}, where the number of training instances are limited to 10$k$. The table header indicates the order of the tasks. Models may perform worse than majority guess because only exact match of generated answer sequences and the ground truth counts as a correct prediction.}
\label{tab:glue}
\end{table*}

==> tables/glue_cl_tab2.tex <==
\begin{table*}[]
\centering
\scalebox{0.7}{
\begin{tabular}{@{}l|rrrrrrrrr|r@{}}
\toprule
\textbf{Task}               & \textbf{CoLA} & \textbf{SST-2} & \textbf{MRPC} & \textbf{STS-B} & \textbf{QQP} & \textbf{MNLI} & \textbf{QNLI} & \textbf{RTE} & \textbf{WNLI} & \textbf{Average} \\ \midrule
%\textit{Continual learning} &      &       &      &       &     &      &      &     &      &         \\
%{BART-LAMOL}              &      &       &      &       &     &      &      &     &      &         \\
%{BART-MBPA}              &   60.40  &   73.74     &    61.27   &   66.47    &  69.50   &   45.56   &  63.31    &   55.96   &   39.44   &    59.52    \\
{BART-Vanilla}              &   77.56  &   88.07     &    80.88   &   84.47    &  80.54   &   71.28   &   83.10    &   59.21   &   43.66   &    74.31  \\

{BART-MbPA++}    &  \smallnum{80.15}    &    \smallnum{91.97}   &        \smallnum{80.64}    &   \smallnum{84.73}    &   \smallnum{83.25}     &    \smallnum{75.50}   &\smallnum{85.56}     &  \smallnum{58.84}    & \smallnum{56.34}      &  \smallnum{77.48}  \\

%             &   30.87    &    70.41   &   68.38   &       49.53 &  67.06    &  32.75     &    76.50   &  62.09   &    43.66   &      55.69   \\
{BART-meta-MbPA}             &   \smallnum{81.69}   &   \smallnum{91.62}    &   \smallnum{82.84}   &    \smallnum{85.53}   &    \smallnum{85.25}  &   \smallnum{75.94}     &    \smallnum{85.25}  & \smallnum{63.18}     &  \smallnum{56.34}    &   \smallnum{78.63}      \\
%         & 0.00     &   49.54    &  31.37    &  49.53     &  63.18   &  0.00  &  63.92     & 70.76 &  56.34  &    42.75     \\ 
{\method-Vanilla}                          & \smallnum{79.70}    &   \smallnum{91.51}     &  \smallnum{84.06}    &   \smallnum{86.20}    &  \smallnum{79.55}   &   \smallnum{77.26}   & \smallnum{87.74}  & \smallnum{71.48} & \smallnum{59.15}     &   \smallnum{79.67}       \\
%{\method-EWC}                &   0.00   & 80.16   &  0.00    &   0.00    &  0.00   &   0.00   &   51.18   &   60.65   &   57.74    &     27.76    \\
\method-EWC                          &   \smallnum{79.70}   & \smallnum{91.74}   &  \smallnum{73.53} &   \smallnum{83.13}    &  \smallnum{81.51}   &   \smallnum{75.42}   &  \smallnum{87.11}    &   \smallnum{70.76} &  \smallnum{57.75} &    \smallnum{77.85}     \\
%{\method-Reg}               &  30.87    &   89.90    &  63.23  &    82.13   &  81.04   &  75.55  &   75.03    &   62.09    & 60.56  &    68.93     \\
{\method-Reg}                             &  \smallnum{79.70}    &   \smallnum{90.94}    &   \smallnum{86.76}    &  \smallnum{85.73}    &  \smallnum{82.43}   &   \smallnum{76.22}    &  \smallnum{86.56}  &   \smallnum{69.68}  &  \smallnum{60.56}  & \smallnum{\textbf{79.84}}   \\
%               &   60.11    &   91.28     &    83.82   &   81.47    &  81.25   &   73.02   &   70.09   &  62.45   &    57.74   &   73.47  \\
{\method$_{\backslash \textrm{ST}}$-Reg}     &   \smallnum{78.04}    &   \smallnum{90.82}     &    \smallnum{86.52}  &    \smallnum{86.00}   &  \smallnum{81.95}   &    \smallnum{75.52}   &  \smallnum{87.06}    &  \smallnum{62.45}   &   \smallnum{57.74}   &     \smallnum{78.46}    \\
%            &   78.72   &   89.68    &   31.62    &    49.80    &  78.98   &    44.38   &   57.66   &  63.54   &    59.15   &     61.50    \\
{HNET$_{d=4}$-Reg}        &   \smallnum{79.19}    &   \smallnum{92.43}     &    \smallnum{70.09}  &    \smallnum{83.20}   &  \smallnum{79.13}   &    \smallnum{75.83}   &  \smallnum{86.40}    &  \smallnum{70.40}   &   \smallnum{59.15}   &     \smallnum{74.01}    \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Performance on GLUE datasets evaluated right after learning a task}. The table header indicates the order of the tasks.}
\label{tab:glue2}
\end{table*}

==> tables/glue_leopard_full.tex <==
\begin{table*}[]
\centering
\scalebox{0.6}{
\begin{tabular}{@{}l|lllllllllllllll|l@{}}
\toprule
\textbf{Task}               & \textbf{CoNLL} & \textbf{MITR} & \textbf{Airline} & \textbf{Disaster} & \textbf{Emotion} & \textbf{P. Bias} & \textbf{P. Audience} & \textbf{P. Message} & \textbf{Books} & \textbf{DVD} & \textbf{Electronics} & \textbf{Kitchen} & \textbf{Scitail} & \textbf{Books R.} & \textbf{Kitchen R.} & \textbf{Average} \\ \midrule
\textbf{N-way}              &                &               &                  &                   &                  &                  &                      &                     &                       &                     &                             &                         &                  &                       &                         &                  \\
\textbf{Continual learning} &                &               &                  &                   &                  &                  &                      &                     &                       &                     &                             &                         &                  &                       &                         &                  \\
\textbf{Vanilla}            &                &               &                  &                   &                  &                  &                      &                     &                       &                     &                             &                         &                  &                       &                         &                  \\
\textbf{EWC}                &                &               &                  &                   &                  &                  &                      &                     &                       &                     &                             &                         &                  &                       &                         &                  \\
\textbf{MAS}                &                &               &                  &                   &                  &                  &                      &                     &                       &                     &                             &                         &                  &                       &                         &                  \\
\textbf{LAMOL}              &                &               &                  &                   &                  &                  &                      &                     &                       &                     &                             &                         &                  &                       &                         &                  \\
\textbf{HNet}               &                &               &                  &                   &                  &                  &                      &                     &                       &                     &                             &                         &                  &                       &                         &                  \\ \midrule
\textbf{Offline learning}   &                &               &                  &                   &                  &                  &                      &                     &                       &                     &                             &                         &                  &                       &                         &                  \\
\textbf{BART-Adapter}       &                &               &                  &                   &                  &                  &                      &                     &                       &                     &                             &                         &                  &                       &                         &                  \\
\textbf{BART-MTL}           &                &               &                  &                   &                  &                  &                      &                     &                       &                     &                             &                         &                  &                       &                         &                  \\
\textbf{BART-Single}        &                &               &                  &                   &                  &                  &                      &                     &                       &                     &                             &                         &                  &                       &                         &                  \\ \bottomrule
\end{tabular}
}
\caption{Few}
\end{table*}

==> tables/glue_leopard_small.tex <==
\begin{table*}[]
\centering
\scalebox{0.7}{
\begin{tabular}{@{}l|cccc|c@{}}
\toprule
\textbf{Task}               & \textbf{Entity Typing} & \textbf{Text Classification} & \textbf{NL Inference} & \textbf{Sentiment Analysis} & \textbf{Average}  \\
\textbf{Task Num.}              & 2                    & 10                           & 1                     & 4                      &  17 \\   \midrule               
\rowcolor{na}  \textit{Continual learning} &                      &                              &                       &                        &                  \\
BART-Vanilla            &       59.57            &          54.21                     &             64.35              &            78.83               &  61.23  \\
BART-MBPA              &        60.88          &               54.39               &           69.59            &          85.58              &       63.39           \\
BART-meta-MbPA              &       63.26         &             54.14             &             71.93          &            84.80            &        63.47          \\
\method-Vanilla            &       67.40       &            58.75                  &         78.46          &        85.83            &           67.30       \\
\method-EWC                &      66.54          &            58.19              &            69.04           &           84.73             &     66.06           \\
%\method-MAS                &                      &                              &                       &                        &                  \\
%BART-LAMOL              &                      &                              &                       &                        &                  \\
\method-Reg               &       66.60          &            58.78                  &            73.75           &         87.88               &  \textbf{67.43}    \\
{\method$_{\backslash \textrm{ST}}$-Reg}         &         61.44          &            57.62                &            68.39           &         84.73             &      65.08
\\ \midrule
\rowcolor{na}  \textit{Single-task learning}   &                      &                             &                       &                        &                  \\

% \textbf{BART-MTL}           &                      &                              &                       &                        &                  \\
HNET-Single        &      64.71            &           56.70           &           57.90           &        71.95           &   61.30 \\
BART-Adapter       &      61.76       &           54.32         &              58.61         &         71.87           &       59.58         
\\ \bottomrule
\end{tabular}
}
\caption{Few shot learning over 17 NLP tasks used in~\cite{Bansal2020LearningTF} grouped by task category. We either uses the model obtained at the end of training on the GLUE task sequence, or train the model from initial BART.}
\label{tab:leopard_few_shot}
\end{table*}

==> tables/kilt_cl.tex <==
\begin{table*}[]
\centering
\scalebox{0.7}{
\begin{tabular}{@{}l|rrrrrrrrr|r@{}}
\toprule
\textbf{Task}               & \textbf{CoLA} & \textbf{SST-2} & \textbf{MRPC} & \textbf{STS-B} & \textbf{QQP} & \textbf{MNLI} & \textbf{QNLI} & \textbf{RTE} & \textbf{WNLI} & \textbf{Average} \\ \midrule
\textit{Continual learning} &      &       &      &       &     &      &      &     &      &         \\
\textbf{Vanilla}            & 0.00     &   53.40    &  31.37    &  0.00     &  63.18   &  35.33  &  49.46     & 43.32 & 60.56  &         \\ 
\addlinespace[-0.1cm]
                            & \smallnum{69.87}    &   \smallnum{91.74}     &  \smallnum{86.03}    &   \smallnum{85.60}    &  \smallnum{81.27}   &   \smallnum{75.86}   & \smallnum{61.12}  & \smallnum{67.87} & \smallnum{60.56}     &         \\
\textbf{EWC}                &   0.00   & 0.01   &  31.62    &   49.53    &  63.18   &   35.33   &   49.46   &  61.01   & 56.33    &         \\
\addlinespace[-0.1cm]
                            &   \smallnum{69.13}   & \smallnum{91.34}   &  \smallnum{87.25} &   \smallnum{86.47}    &  \smallnum{83.28}   &   \smallnum{76.21}   &  \smallnum{61.03}    &   \smallnum{71.48} &  \smallnum{56.33} &         \\
\textbf{MAS}                &      &       &      &       &     &      &      &     &      &         \\
\textbf{LAMOL}              &      &       &      &       &     &      &      &     &      &         \\
\textbf{HNet}               &  69.13    &   89.10    &  78.43  &    85.20   &  64.67   &  57.54  &   49.46    &   56.32    &  60.56  &         \\
\addlinespace[-0.1cm]
                            &  \smallnum{69.13}    &   \smallnum{89.56}    &   \smallnum{86.27}    &  \smallnum{85.60}    &  \smallnum{82.79}   &   \smallnum{76.98}    &  \smallnum{61.27}  &   \smallnum{74.37}  &  \smallnum{60.56}  &  \\
\midrule
\textit{Offline learning}   &       &       &      &       &     &      &      &     &      &         \\
\textbf{HNet-Single}       &   69.13   &   92.08    &   85.54    &   85.00      &  82.31   &   75.78   &   59.53    &   ?  &   ?   &         \\
\textbf{Adapter-Single}    &   69.13   &   91.28   &   77.94   &    84.20   &  82.53   &   75.19   &  60.52  &  ?   &   ?   &         \\
\textbf{BART-Single}        &      &       &      &       &     &      &      &     &      &         \\ 
\textbf{BART-MTL}           &      &       &      &       &     &      &      &     &      &         \\
\bottomrule
\end{tabular}
}
\caption{Continual and offline learning performance on KILT datasets. For the CL setup, the numbers above are evaluated at the end of the training; while numbers below are evaluated right after learning the task. The table header also indicates the order of the tasks.}
\end{table*}

==> tables/new/final_performance.tex <==
\begin{table}[]
\centering
\scalebox{0.66}{
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{tabular}{@{}lcc@{}}
\toprule
%\textbf{Task}                 & \textbf{All}    \\
             &  \textbf{GLUE} & \textbf{CrossFit-Cls-Train}    \\ \midrule
\rowcolor{na}  \textit{Continual learning}   &       &        \\
BART-Vanilla                  &         &     $50.42$                 \\
BART-EWC                      &         &          \\
BART-MbPA++                   &         &                    \\
\rowcolor{na} \textit{Continual meta-learning}       &              &               \\
BART-meta-MbPA                &                &                  \\
\method-Vanilla               &           & $64.97_{\pm 2.1}$                    \\
\method-EWC                   &         &        \\
\method-Reg                   &         & $68.23_{\pm 2.1}$         \\
 \rowcolor{na} Single Task-Learning          &      &          \\
 BART-Single                &               &           \\
\method-Single                &              &                         \\
\rowcolor{na} Multi-Task Learning  &          &           \\
BART-MTL                     &                 &                          \\
\method~MTL                   &         &     66.15$_{\pm 4.3}$                         \\
Majority                      &         &          \\ \bottomrule
\end{tabular}
}
\caption{Model performance measured at the end of training (Final Acc.) on GLUE and CrossFit-Cls training tasks.}
\end{table}

==> tables/new/instant_performance.tex <==
\begin{table}[]
\centering
\scalebox{0.66}{
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{tabular}{@{}lcc@{}}
\toprule
%\textbf{Task}                 & \textbf{All}    \\
             &  \textbf{GLUE} & \textbf{CrossFit-Cls-Train}    \\ \midrule
\rowcolor{na}  \textit{Continual learning}   &       &        \\
BART-Vanilla                  &         &     $50.42$                 \\
BART-EWC                      &         &          \\
BART-MbPA++                   &         &                    \\
\rowcolor{na} \textit{Continual meta-learning}       &              &               \\
BART-meta-MbPA                &                &                  \\
\method-Vanilla               &           & $64.97_{\pm 2.1}$                    \\
\method-EWC                   &         &        \\
\method-Reg                   &         & $68.23_{\pm 2.1}$         \\
 \rowcolor{na} Single Task-Learning          &      &          \\
 BART-Single                &               &           \\
\method-Single                &              &                         \\
\rowcolor{na} Multi-Task Learning  &          &           \\
BART-MTL                     &                 &                          \\
\method~MTL                   &         &     66.15$_{\pm 4.3}$                         \\
Majority                      &         &          \\ \bottomrule
\end{tabular}
}
\caption{Model performance measured right after learning each task (Instant Acc.) on GLUE and CrossFit-Cls training tasks.}
\end{table}

==> tables/text_classification_cl.tex <==
\begin{table}[]
\centering
\scalebox{0.6}{
\begin{tabular}{@{}l|ccccc@{}}
\toprule
\textbf{Order} & \textbf{MbPA} & \textbf{Meta-MbPA} & \textbf{LAMOL} & \textbf{HNET-Reg} & \textbf{HNET$_{d=3}$-Reg} \\ \midrule
i.             & 75.3                 & 77.9                          & 76.7           & 75.1   &   73.4        \\
ii.            & 74.6                 & 76.7                          & 77.2           & 73.8   &   73.6    \\
iii.           & 75.6                 & 77.3                          & 76.1           & 74.8   &   68.3        \\
iv.            & 75.5                 & 77.6                          & 76.1           & 73.9   &   73.7    \\ \midrule
Average        & 75.3                 & 77.3                          & 76.5           & 74.4   &     72.7      \\ 
MTL Avg.            & 78.9                 & 78.9                          & 78.9           & 74.4      &    74.4    \\ \midrule
Diff.          & -3.6                  & -1.6                           & -2.4            & 0.0     &     -1.7     \\ \bottomrule
\end{tabular}
}
\caption{Continual and multi-task learning (MTL) performance over four text classification tasks over four different orders. The results of MbPA++, Meta-MbPA, and LAMOL are cited from~\cite{Wang2020EfficientML} and use a different model architecture, and thus numbers are not directly comparable. We also show differences between the corresponding MTL and CL performance.}
\label{tab:cl_text_cls}
\end{table}
